LinkMirage: How to Anonymize Links in Dynamic Social Systems

Social network based trust relationships present a critical foundation for designing trustworthy systems, such as Sybil defenses, secure routing, and anonymous/censorshipresilient communications. A key issue in the design of such systems, is the revelation of users' trusted social contacts to an adversary-information that is considered sensitive in today's society. In this work, we focus on the challenge of preserving the privacy of users' social contacts, while still enabling the design of social trust based applications. First, we propose LinkMirage, a community detection based algorithm for anonymizing links in social network topologies; LinkMirage preserves community structures in the social topology while anonymizing links within the communities. LinkMirage considers the evolution of the social network topologies, and minimizes privacy leakage due to temporal dynamics of the system. Second, we define metrics for quantifying the privacy and utility of a time series of social topologies with anonymized links. We analyze the privacy and utility provided by LinkMirage both theoretically, as well as using real world social network topologies: a Facebook dataset with 870K links and a large-scale Google+ dataset with 940M links. We find that our approach significantly outperforms the existing state-of-art. Finally, we demonstrate the applicability of LinkMirage in real-world applications such as Sybil defenses, reputation systems, anonymity systems and vertex anonymity. We also prototype LinkMirage as a Facebook application such that real world systems can bootstrap privacy-preserving trust relationships without the cooperation of the OSN operators.

==> temporal.tex <==
\subsection{temporal situation}

Considering a Gauss-Markov process, where
\begin{equation}
\begin{aligned}
&{\bf{x}}_{t+1}={\bf{A}}_t{\bf{x}}_t+{\bf{w}}_t, t=0,1,\cdots,T-1\\
&{\bf{w}}_t\sim\mathcal{N}(0,{\bf W}_t), \bf{w}_t \mathrm{ is independent of } \bf{x}_0, \bf{w}^{t-1}
\end{aligned}
\end{equation}
where ${\bf{w}}^{t-1}=\left({\bf{w}}_0, \cdots, {\bf{w}}_{t-1}\right)$
The Gaussian SRD (sequential rate distortion) problem is
\begin{equation}
\sum_{t=1}^T I(\bf{x}^t, \bf{z}|\bf{z}^{t-1})+\frac{\alpha_t}{2}\mathbb{E}\|\bf{x}_t-\bf{z}_t\|^2
\end{equation}
Replacing $\bf{z}$ with $\hat{\bf{x}}$, we have
\begin{equation}
\sum_{t=1}^T I(\bf{x}^t, \hat{\bf{x}}_t|\hat{\bf{x}}^{t-1})+\frac{\alpha_t}{2}\mathbb{E}\|\bf{x}_t-\hat{\bf{x}}_t\|^2
\end{equation}

\begin{figure}[!t]
\centering
\includegraphics[width=3.3in,height=1in]{temporal.eps}
\DeclareGraphicsExtensions.
\caption{Perturbation scheme for the Gaussian Markov sources.}
\label{perturb_tempo}
\end{figure}


\begin{algorithm}[!t]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand\algorithmicensure {\textbf{Output:}}
\begin{algorithmic}[1]
\REQUIRE~~{$G_1, G_2, \cdots, G_T, D, \epsilon$}\\
\ENSURE  {$G_1^\prime, G_2^\prime, \cdots, G_T^\prime$};\\
       $\left\{G_i^{\prime}\right\}=$null;\\
       compute the transition matrix $\bf{A}$ according to Eq.(\ref{transition});\\
       compute the noise covariance matrix $\bf{W}$ according to Eq.(\ref{noiseCM});\\
       compute the optimal matrix $\bf{P}, \bf{Q}$ according to Eq.(\ref{sta_opt});\\
       design the sensing matrix $\bf{C}, \bf{V}$ according to Eq.(\ref{CV});\\
       \textbf{foreach} temporal graph $G_t$\\
       $~~~$ \textbf{foreach} close node pair $(u,v)$ in $G_t$\\
       $~~~~~~$ compute the original affinity score $w_{(t)uv}$;\\
       $~~~$ construct the input sequence as ${\bf{w}}_t=\{w_{(t)uv}\}$\\
       $~~~$ compute the sensing output $\bf{y}^t$ according to Eq.(\ref{sensing});\\
       $~~~$ kalman filter $\bf{y}_t$ to obtain $\bf{\hat{x}}_t=\mathbb{E}(\bf{x}_t|\bf{y}_t)$;\\
       $~~~$ \textbf{foreach} close node pair $(u,v)$\\
       $~~~~~~$ \textbf{if} $w^{\prime}_{uv}>\epsilon$\\
       $~~~~~~~~~$ add edge $(u,v)$ to $G^\prime_t$;\\
       return $G_1^\prime, G_2^\prime, \cdots, G_T^\prime$;\\
\caption{Perturb graph series $G_1, G_2, \cdots, G_T$ with optimal privacy under distortion $D$.}
\label{gaussian_per_temporal}
\end{algorithmic}
\end{algorithm}

\cite{Tanaka:arxiv} is proven that this SRD problem is equivalent to the linear Gaussian sensor (LGS) design problem.
The sensing process is
\begin{equation}\label{sensing}
\bf{y}_t=\bf{C}_t\bf{x}_t+\bf{v}_t
\end{equation}

\begin{equation}
\begin{aligned}
\min_{\{\bf{C}_t,\bf{V}_t\}_{t=1}^T} &\sum_{t=1}^T I(\bf{x}_t, \bf{y}_t | \bf{y}^{t-1})+\frac{\alpha_t}{2}\mathbb{E}\|\bf{x}_t-\hat\bf{x}_t\|^2\\
& \mathrm{s.t.~} \bf{y}_t=\bf{C}_t\bf{x}_t+\bf{V}_t, \bf{V}_t\sim\mathcal{N}(0,\bf{V}_t)\\
& \bf{v}_t \mathrm{~is~independent~of~} \bf{x}_0, \bf{w}^t, \bf{V}^{t-1}\\
& \bf{\hat{x}}_t=\mathbb{E}\left(\bf{x}_t|\bf{y}^t\right)
\end{aligned}
\end{equation}

where the Kalman filter is to find $\bf{\hat{x}}_t=\mathbb{E}\left(\bf{x}_t|\bf{y}^t\right)$. And the detailed process is
\begin{equation}
\begin{aligned}
&\bf{\hat{x}}_t=\bf{\hat{x}}_{t|t-1}+\bf{P}_{t|t-1}\bf{C}_t^T\left(\bf{C}_t\bf{P}_{t|t-1}\bf{C}_{t}^T+\bf{V}_t\right)^{-1}\left(\bf{y}_t-\bf{C}_t\bf{\hat{x}}_{t|t-1}\right)\\
&\bf{\hat{x}}_{t|t-1}=\bf{A}_{t-1}\bf{\hat{x}}_{t-1}\\
&\bf{P}_{t|t-1}=\bf{A}_{t-1}\bf{P}_{t-1|t-1}\bf{A}^T_{t-1}+\bf{W}_{t-1}\\
&\bf{P}_{t|t}=\left(\bf{P}_{t|t-1}^{-1}+\bf{C}_t^T\bf{V}_t^{-1}\bf{C}_t\right)\\
\end{aligned}
\end{equation}
and
\begin{equation}\label{CV}
\bf{C}_t^T\bf{V}_t^{-1}\bf{C}_t=\bf{P}_{t|t}^{-1}-\left(\bf{A}_{t-1}\bf{P}_{t-1|t-1}\bf{A}_{t-1}^T+\bf{W}_{t-1}\right)^{-1}
\end{equation}
Considering the stationary case where $\bf{A}_t, \bf{W}_t, \bf{P}_{t|t}, \bf{Q}_t$ are time-invariant.

Then, it is equivalent to solve
\begin{equation}\label{sta_opt}
\begin{aligned}
&\min_{\bf{P}, \bf{Q}} -\frac{1}{2}\log\det \bf{Q}+\frac{1}{2}\log\det \bf{W}\\
&\mathrm{s.t.~} \bf{Q}\succ \bf{0}\\
& \bf{P}\preceq \bf{A}\bf{P}\bf{A}^T+\bf{W}\\
& Tr(\bf{P})\leq 0\\
&\left[\begin{array}{ll}
\bf{P}-\bf{Q} & \bf{PA^T} \\
\bf{AP} & \bf{APA^T+W} \\
\end{array} \right]\succeq \bf{0}
\end{aligned}
\end{equation}

However, given a sequence of temporal graphs $G^T=[G_1, G_2, \cdots, G_T]$, we have to first estimate the matrix $\bf{A}$ and $\bf{W}$.
According to the maximum-likelihood theory, we can estimate the matrix as
\begin{equation}\label{transition}
\begin{aligned}
&\min_{\bf{A}} \sum_{t=2}^T\|\bf{x}_t-\bf{A}\bf{x}_{t-1}\|^2\\
&=\min_{\bf{A}} \|\bf{X}_2-\bf{A}\bf{X}_1\|^2
\end{aligned}
\end{equation}
where
\begin{equation}\label{noiseCM}
\begin{aligned}
\bf{X}_2&=[\bf{x}_2,\cdots,\bf{x}_T]\\
\bf{X}_1&=[\bf{x}_1,\cdots,\bf{x}_{T-1}]
\end{aligned}
\end{equation}
Then, we have
\begin{equation}
W=\frac{1}{T}\sum_{t=1}^T \mathrm{diag}\left\{(\bf{x}_t-\bf{A}\bf{x}_t)^T(\bf{x}_t-\bf{A}\bf{x}_t)\right\}
\end{equation}



\begin{figure*}[!t]
\centering
\subfigure[]{
\label{MIber} %% label for first subfigure
\includegraphics[width=3.5in,height=1.7in]{RDtempora.eps}}
\subfigure[]{
\label{ratioBernouli} %% label for second subfigure
\includegraphics[width=3.5in,height=1.7in]{ratio_tempora.eps}}
\caption{Mutual Information vs Statistical Utility Distance \& Ratio of Overlapped Edges vs Statistical Utility Distance for temporal Gaussian distribution.}
\label{ber} %% label for entire figure
\end{figure*}
